Reinforcement Learning-based Dialogue Guided Event Extraction to Exploit Argument Relations

Event extraction is a fundamental task for natural language processing. Finding the roles of event arguments like event participants is essential for event extraction. However, doing so for real-life event descriptions is challenging because an argument's role often varies in different contexts. While the relationship and interactions between multiple arguments are useful for settling the argument roles, such information is largely ignored by existing approaches. This paper presents a better approach for event extraction by explicitly utilizing the relationships of event arguments. We achieve this through a carefully designed task-oriented dialogue system. To model the argument relation, we employ reinforcement learning and incremental learning to extract multiple arguments via a multi-turned, iterative process. Our approach leverages knowledge of the already extracted arguments of the same sentence to determine the role of arguments that would be difficult to decide individually. It then uses the newly obtained information to improve the decisions of previously extracted arguments. This two-way feedback process allows us to exploit the argument relations to effectively settle argument roles, leading to better sentence understanding and event extraction. Experimental results show that our approach consistently outperforms seven state-of-the-art event extraction methods for the classification of events and argument role and argument identification.

==> 10-beifen.tex <==

\begin{table*}[!htbp]
\centering
\caption{The P (precision), R (recall), and F1 score on  event classification, argument identification and argument role classification results performed on the ACE2005 testset. 
Best results are highlighted in bold and ``–" means results are not available. 
%The dialogue guided model includes the two keys innovation: incremental event learning and reinforcement learning guided dialogue.
% The full model adds the lexicon-based GAT and multi-task learning module.
}
\label{ACE2005}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
\textbf{Task} & \multicolumn{3}{l}{\textbf{Event Classification (\%)}} & \multicolumn{3}{|l}{\textbf{Argument Identification (\%)}} & \multicolumn{3}{|l}{\textbf{Argument Role Classification (\%)}}  \\
 & P   & R   & F1  & P  & R & F1  & P  & R & F1  \\\midrule
DBRNN \cite{DBLP:conf/aaai/ShaQCS18} & 74.10  & 69.80  & 71.90 &71.30&64.50&67.70 & 66.20  & 52.80  & 58.70  \\
JMEE \cite{DBLP:conf/emnlp/LiuLH18} & 76.10  & 71.30  & 73.70 &71.40&\textbf{65.60}&68.40& 66.80  & 54.90  & 60.30  \\
Joint3EE \cite{DBLP:conf/aaai/NguyenN19} & 68.00  & 71.80  & 69.80  &59.90&59.80&69.90& 52.10  & 52.10  & 52.10 \\
GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} &   74.80  & 69.40 & 72.0  &63.30&48.70& 55.10  & 61.60  &  45.70  &  52.40     \\
PLMEE \cite{DBLP:conf/acl/YangFQKL19} &   81.00  & 80.40 & 80.70&71.40&60.10& 65.30  & 62.30  &  54.20  & 58.00   \\
% Chen et al. \cite{DBLP:journals/corr/abs-1912-01586}& 66.7   &  74.7  & 70.5 &44.9 &41.2&43.0& 44.3 & 40.7  & 42.4  \\\hline
Du et al. \cite{DBLP:conf/emnlp/DuC20} &  71.12  &  73.70  &72.39 &58.9&52.08&55.29 & 56.77 & 50.24  &53.31    \\
MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20} &  -  &  -  &73.8 &-&-&56.7 & - & - &55.0    \\
\hline 
\rowcolor{Gray} Our fine-tuned BERT &  79.81  & 79.62   & 79.96&70.42&60.24& 64.12 & 62.34 & 53.45  &  57.80  \\
% \hline    
\rowcolor{Gray} Our dialogue guided model &  82.25  & 80.70  & 81.33&72.75&63.53& 67.71 & 67.67 & \textbf{54.92}  &  59.42  \\
\rowcolor{Gray} Our full model &  \textbf{84.34}  & \textbf{81.96}   & \textbf{83.37}&\textbf{73.43}&65.30& \textbf{69.97} & \textbf{69.82} & 54.43  &  \textbf{61.42}  \\\bottomrule
\end{tabular}
}
\end{table*}






\begin{table*}[!htbp]
\centering
\caption{The P (precision), R (recall), and F1 score on  event classification, argument identification and argument role classification results performed on the KBP  testset. 
Best results are highlighted in bold and ``–" means results are not available. 
%The dialogue guided model includes the two keys innovation: incremental event learning and reinforcement learning guided dialogue.
% The full model adds the lexicon-based GAT and multi-task learning module.
}
\label{KBP}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
\textbf{Task} & \multicolumn{3}{l}{\textbf{Event Classification (\%)}} & \multicolumn{3}{|l}{\textbf{Argument Identification (\%)}} & \multicolumn{3}{|l}{\textbf{Argument Role Classification (\%)}}  \\
 & P   & R   & F1  & P  & R & F1  & P  & R & F1  \\\midrule
DBRNN \cite{DBLP:conf/aaai/ShaQCS18} & 74.10  & 69.80  & 71.90 &71.30&64.50&67.70 & 66.20  & 52.80  & 58.70  \\
JMEE \cite{DBLP:conf/emnlp/LiuLH18} & 76.10  & 71.30  & 73.70 &71.40&\textbf{65.60}&68.40& 66.80  & 54.90  & 60.30  \\
Joint3EE \cite{DBLP:conf/aaai/NguyenN19} & 68.00  & 71.80  & 69.80  &59.90&59.80&69.90& 52.10  & 52.10  & 52.10 \\
GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} &   74.80  & 69.40 & 72.0  &63.30&48.70& 55.10  & 61.60  &  45.70  &  52.40     \\
PLMEE \cite{DBLP:conf/acl/YangFQKL19} &   81.00  & 80.40 & 80.70&71.40&60.10& 65.30  & 62.30  &  54.20  & 58.00   \\
% Chen et al. \cite{DBLP:journals/corr/abs-1912-01586}& 66.7   &  74.7  & 70.5 &44.9 &41.2&43.0& 44.3 & 40.7  & 42.4  \\\hline
Du et al. \cite{DBLP:conf/emnlp/DuC20} &  71.12  &  73.70  &72.39 &58.9&52.08&55.29 & 56.77 & 50.24  &53.31    \\
MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20} &  -  &  -  &73.8 &-&-&56.7 & - & - &55.0    \\
\hline 
\rowcolor{Gray} Our fine-tuned BERT &  79.81  & 79.62   & 79.96&70.42&60.24& 64.12 & 62.34 & 53.45  &  57.80  \\
% \hline    
\rowcolor{Gray} Our dialogue guided model &  82.25  & 80.70  & 81.33&72.75&63.53& 67.71 & 67.67 & \textbf{54.92}  &  59.42  \\
\rowcolor{Gray} Our full model &  \textbf{84.34}  & \textbf{81.96}   & \textbf{83.37}&\textbf{73.43}&65.30& \textbf{69.97} & \textbf{69.82} & 54.43  &  \textbf{61.42}  \\\bottomrule
\end{tabular}
}
\end{table*}






\begin{table*}[!htbp]
\centering
\caption{The P (precision), R (recall), and F1 score on  event classification, argument identification and argument role classification results performed on the ACE2005 testset. 
Best results are highlighted in bold and ``–" means results are not available. 
%The dialogue guided model includes the two keys innovation: incremental event learning and reinforcement learning guided dialogue.
% The full model adds the lexicon-based GAT and multi-task learning module.
}
\label{ACE2005}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrr|rrr}
\toprule
\textbf{Task} & \multicolumn{3}{l}{\textbf{Event Classification (\%)}} & \multicolumn{3}{l}{\textbf{Trigger Identification (\%)}}  \\
 & Precision   & Recall   & F1 & Precision   & Recall   & F1   \\\midrule
DBRNN \cite{DBLP:conf/aaai/ShaQCS18} & 74.10  & 69.80  & 71.90 & & &   \\
JMEE \cite{DBLP:conf/emnlp/LiuLH18} & 76.10  & 71.30  & 73.70 & & &  \\
Joint3EE \cite{DBLP:conf/aaai/NguyenN19} & 68.00  & 71.80  & 69.80  & & &   \\
GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} &   74.80  & 69.40 & 72.0  & & &       \\
PLMEE \cite{DBLP:conf/acl/YangFQKL19} &   81.00  & 80.40 & 80.70& & &      \\
% Chen et al. \cite{DBLP:journals/corr/abs-1912-01586}& 66.7   &  74.7  & 70.5 &44.9 &41.2&43.0& 44.3 & 40.7  & 42.4  \\\hline
Du et al. \cite{DBLP:conf/emnlp/DuC20} &  71.12  &  73.70  &72.39 & & &      \\
MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20} &  -  &  -  &73.8 &-&-&    \\
\hline 
\rowcolor{Gray} Our fine-tuned BERT &  79.81  & 79.62   & 79.96& & &      \\
% \hline    
\rowcolor{Gray} Our dialogue guided model &  82.25  & 80.70  & 81.33& & &    \\
\rowcolor{Gray} Our full model &  \textbf{84.34}  & \textbf{81.96}   & \textbf{83.37}& & &   \\\bottomrule
\end{tabular}
}
\end{table*}




\begin{table*}[!htbp]
\centering
\caption{The P (precision), R (recall), and F1 score on  event classification, argument identification and argument role classification results performed on the KBP  testset. 
Best results are highlighted in bold and ``–" means results are not available. 
%The dialogue guided model includes the two keys innovation: incremental event learning and reinforcement learning guided dialogue.
% The full model adds the lexicon-based GAT and multi-task learning module.
}
\label{KBP}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrr|rrr}
\toprule
\textbf{Task} & \multicolumn{3}{|l}{\textbf{Argument Identification (\%)}} & \multicolumn{3}{|l}{\textbf{Argument Role Classification (\%)}}  \\
 &  Precision  & Recall & F1  & Precision  & Recall & F1  \\\midrule
DBRNN \cite{DBLP:conf/aaai/ShaQCS18} &71.30&64.50&67.70 & 66.20  & 52.80  & 58.70  \\
JMEE \cite{DBLP:conf/emnlp/LiuLH18} &71.40&\textbf{65.60}&68.40& 66.80  & 54.90  & 60.30  \\
Joint3EE \cite{DBLP:conf/aaai/NguyenN19} &59.90&59.80&69.90& 52.10  & 52.10  & 52.10 \\
GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} &63.30&48.70& 55.10  & 61.60  &  45.70  &  52.40     \\
PLMEE \cite{DBLP:conf/acl/YangFQKL19} &71.40&60.10& 65.30  & 62.30  &  54.20  & 58.00   \\
% Chen et al. \cite{DBLP:journals/corr/abs-1912-01586}& 66.7   &  74.7  & 70.5 &44.9 &41.2&43.0& 44.3 & 40.7  & 42.4  \\\hline
Du et al. \cite{DBLP:conf/emnlp/DuC20} &58.9&52.08&55.29 & 56.77 & 50.24  &53.31    \\
MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20} &-&-&56.7 & - & - &55.0    \\
\hline 
\rowcolor{Gray} Our fine-tuned BERT &70.42&60.24& 64.12 & 62.34 & 53.45  &  57.80  \\
% \hline    
\rowcolor{Gray} Our dialogue guided model &72.75&63.53& 67.71 & 67.67 & \textbf{54.92}  &  59.42  \\
\rowcolor{Gray} Our full model &\textbf{73.43}&65.30& \textbf{69.97} & \textbf{69.82} & 54.43  &  \textbf{61.42}  \\\bottomrule
\end{tabular}
}
\end{table*}




\begin{table}[t]
\centering
\caption{Ablation study on Global Constraints on F1-score (\%).}
\label{Ablation}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Tasks} & \textbf{Ours} &  \textbf{-RLD} & \textbf{-IEL} & \textbf{-LGAT}   & \textbf{-MTL}  \\ 
\midrule
EC  & \textbf{83.37} & 83.37 & 81.25 &  82.96   &81.33   \\ 
AI  & \textbf{69.97} &67.12    & 67.63  & 69.45    &  67.72  \\ 
RC & \textbf{61.42}  &59.80 & 60.78 &61.01        &60.22 \\ 
\bottomrule
\end{tabular}
\end{table}


As a departure from prior work, we formulate event extraction within a task-oriented dialogue system \cite{DBLP:conf/aaai/LiptonLG00D18,DBLP:conf/acl/ZhangLGC19}.
It can utilize multi-turn dialogue to extract arguments one by one, which is easy to introduce existing knowledge to the current dialogue.
Furthermore, we use reinforcement learning to rank the order of arguments to maximum utilizing the relation. 
It can use the correlation between arguments by constructing the multiple candidate content based on the event type and the predicted event argument with a high reward to identify the next argument.
On our motivation example $S1$, given the event type ``Conflict: Attack", the best role extraction order is extracting ``Instrument" and ``trigger" before``Attacker" and ``Target".

Figure \ref{exampleACE} shows an example having the same trigger under different positions on two event types.
Figure \ref{exampleACE2} gives the extraction order of argument roles, with the order in bold is the best choice, avoiding extracting the word playing multiple roles first. 
If we can find the best order to maximize the correlation, the result of argument extraction will be more complete and accurate.

This work consider the event extraction task a task-oriented dialogue task \cite{DBLP:conf/aaai/LiptonLG00D18} \cite{DBLP:conf/acl/ZhangLGC19} that aims to accomplish all argument identification and classification under different event types.
The dialogue-based method takes advantage of this relationship, which identifies the current argument by adding existing dialogue to the current dialogue.
Our key insight was using reinforcement learning to learn the ranking policy for dialogue-based argument extraction.
It can use the correlation between arguments by constructing the multiple candidate content based on the event type and the predicted event argument with a high reward to identify the next argument.
Figure \ref{exampleACE} shows an example having the same trigger under different positions on two event types.
Figure \ref{exampleACE2} gives the extraction order of argument roles, with the order in bold is the best choice, avoiding extracting the word playing multiple roles first. 
If we can find the best order to maximize the correlation, the result of argument extraction will be more complete and accurate.



A task-oriented dialogue system can use the dialogue historical information to optimize slot filling order. It has the advantage of modeling order knowledge compared to question answering and sequence labeling. 
In this work, we formulate event extraction within a task-oriented dialogue system. It can be seen as a multi-turn dialogue between two agents, aiming to fill all slots, which is the argument in event extraction. 
For each turn, the \emph{agent A} selects a role and generates content through a dialogue generator. The \emph{agent B} generates content to answer \emph{agent A}. We utilize multi-turn dialogue to extract individual arguments at a time and introduce existing knowledge to the current dialogue. 



Since our model extracts arguments one by one, the extraction of the first argument is crucial.
We present a lexicon-based graph attention network and an event-based BERT model for learning the event representation, exploiting the grammar and semantic knowledge tokens learned.
Furthermore, to introduce argument relations for event representation, we design an incremental learning method to update the event representation and our lexicon-based graph, introducing predicted argument for the next argument extraction.

However, the reinforcement learning based dialogue guided argument extraction needs lots of training data. It is hard to use existing data enhancement methods, such as back-translation \cite{doi:10.1177/135910457000100301} and synonym replacement \cite{DBLP:conf/acl-pitr/AbrahamssonFSK14}.
We design an incremental event learning method to update the event representation and the lexicon-based graph, using the predictive argument to help event classification.
We design an incremental learning method to update the event representation and our lexicon-based graph, introducing predicted argument for the next argument extraction.
Our lexicon-based graph can utilize the  
We design an incremental event learning method, which uses the predictive argument to help event classification.

We present a lexicon-based graph attention network and an event-based BERT model for learning the event representation on event classification and argument extraction, exploiting the grammar and semantic knowledge tokens learned. 
In the motivation example, the sentence ``S1" is a \emph{Conflict: Attack} event, which can be identified through the argument ``weapons" and the trigger ``use" together.
It means the argument can make positive beneficial for event classification.
Moreover, we use the dialogue generation method to produce more training data by generating multiple dialogues for each argument.
As a result, it eliminates the insufficient training data on event extraction tasks.


% \FIXME{This is out of blue. We need to connect this better with the previous paragraph. Why do we need these lexicon-based GCN and BERT models? What are their relationship with the dialogue system? }

% We also design a multi-task model for event classification to overcome event type imbalance results in a low recall. 
We estimate our approach by implementing it to sentence-level event extraction. 
We have accompanied intensive experiments on the ACE 2005 dataset \cite{DBLP:conf/lrec/DoddingtonMPRSW04}.
Our experimental results confirm that ranking the argument extracting order is often sufficient to utilize the relation among arguments by our reinforcement learning-based dialogue framework.
Employing the lexicon-based graph attention network can utilize the argument associating to capture event-level knowledge.  
Furthermore, we show that our model can achieve significant performance improvement under little labeled data via implementing incremental event learning methods.



==> 4-EventRepresentation.tex <==


\section{Event Representation}
\label{sec:EventRepresentation}

The first step of our argument extraction pipeline is to learn the representation (or embeddings) to be used for argument selection. We do so by first constructing a lexicon-based graph, from which we learn the lexicon-based representation of individual words. We then learn the context representation at the sentence-level across multiple words. 
To that end, we use both a lexicon-based graph attention network \cite{DBLP:conf/emnlp/GuiZZPFWH19} and an event-based BERT model \cite{DBLP:conf/nips/VaswaniSPUJGKP17} for learning the word representation from semantics and context perspectives. 

\subsection{Lexicon-based Representation} 

Lexicon-based graph neural network has been designed for the node classification task \cite{DBLP:conf/emnlp/GuiZZPFWH19}, proved to be an effective way to learn global semantics.
Thus, we use lexical knowledge to concatenate characters capturing the local composition and a global relay node to capture long-range dependency.

We convert the sentence to a directed graph (as shown in Fig.~\ref{graph}) where each word is represented as a graph node, and a graph edge represents one of the five relations: words in a lexicon; lexicon to lexicon; a relay node connecting to all nodes; co-occurrence words; and pseudo relation among arguments of an event. 
The first connects words in the phrase sequentially until the last word.
The second is to create a line between phrases that the last word of the current phrase is connected with the latter phrase, and each edge represents the potential characteristics of the word that may exist.
We also use a relay node as a virtual hub, which is connected to all other nodes. 
It gathers all the edges and nodes' information, eliminating the boundary ambiguity between words, and learning long-range dependency.
Therefore, the representation of the relay node can be regarded as the representation of the text.
The fourth edge represents pseudo argument relation by connecting the predicted arguments in an event.
The last one is calculating the co-occurrence probability of words within sliding windows in the corpus.
The edge weights are measured by Pointwise Mutual Information (PMI):
\begin{equation}
% \small
\operatorname{PMI}\left(w_{i}, w_{j}\right)=\log \frac{p(w_{i}, w_{j})}{p(w_{i}) p(w_{j})}=\log \frac{N_{w_{i}, w_{j}} N}{N_{w_{i}} N_{w_{j}}},   \label{eq:r1}
\end{equation}
where $N_{w_{i}}, N_{w_{j}}, N_{w_{i}, w_{j}}$ are the number of sliding windows containing word $w_{i}$, $w_{j}$ and both $w_{i}$, $w_{j}$. $N$ is the total number of sliding windows in the corpus.


To learn the word-level representation, we extend the Lexicon-based Graph Attention Network (LGAT) that is designed for learning global semantics for node classification \cite{DBLP:conf/emnlp/GuiZZPFWH19}. We extend the LGAT by adding a pseudo edge, i.e., by appending an edge among predicted arguments of an event type. Our goal is to update word representation using existing prediction results.
Given an N-word text $T=\{{T_{1}, T_{2}, \dots, T_{N}}\}$, the model embeds the initial input text $ET=\{{ET_{1}, ET_{2}, \dots, ET_{N}}\}$ through the pre-trained embedding matrix. The embedding of predicted event role $R=\{R_{1}, R_{2}, \dots, R_{N}\}$ is represented as $ER=\{ER_{1}, ER_{2}, \dots, ER_{N}\}$. The model takes as input $EI=ET \oplus ER$ and produces a hidden representation $H^{n}=\{{h^{n}_{1}, h^{n}_{2}, \dots, h^{n}_{N}}\}$, for text $T$. Here, $h^{n}_{i}$ represents the text feature of the $i$-th word on the $n$-th hidden layer.
Therefore, the final node representation is: 
\begin{equation}
% \small
{LT}_{i}=f(H^{N}_{i}), i=0, 1, 2, \dots, N, \label{eq:r2}
\end{equation}
where ${LT}_{0}$ is the relay node used to predict the event type.
It is then used to obtain the optimal decision through the Conditional Random Field (CRF).
The probability of a label sequence $\hat{y}=\hat{c_{1}}, \hat{c_{2}}, \dots, \hat{c_{k}}$ can be defined as follows:
\begin{equation}
\phi\left(\hat{c}_{i-1}, \hat{c}_{i}, \mathbf{h}\right)=\mathbf{W}_{\left(c_{i-1}, c_{i}\right)} \mathbf{c}_{i}^{T}+\mathbf{b}_{\left(c_{i-1}, c_{i}\right)}
\end{equation}
where $L(s)$ is the set of all arbitrary label sequences.


% $\phi\left(\hat{c}_{i-1}, \hat{c}_{i}, \mathbf{h}\right)=\mathbf{W}_{\left(c_{i-1}, c_{i}\right)} \mathbf{c}_{i}^{T}+\mathbf{b}_{\left(c_{i-1}, c_{i}\right)}$, 
where $\mathbf{W}_{\left(c_{i-1}, c_{i}\right)}\in \mathbb{R}^{k \times n}$ and $\mathbf{b}_{\left(c_{i-1}, c_{i}\right)}\in \mathbb{R}^{k \times n}$ are the weight and bias parameters specific to the labels $c_{i-1}$ and $c_{i}$, where $k$ is the number of event types, $n$ is the input length of text.

 
 




\subsection{Event-based Context Representation} 
BERT is a multi-layer bidirectional Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17}, achieving significant performance improvement on event extraction task \cite{DBLP:conf/acl/YangFQKL19}.
We use a BERT model \cite{DBLP:conf/acl/YangFQKL19} to learn the context representation. 
Specifically, we feed the sentence text into an event-based BERT model to encode the input text $T$, the predicted event role $R$, and the embedding of \emph{Agent A} (used for dialogue generation described in Section \ref{sec:DialogueGeneration}) $EA=\{EA_{1}, EA_{2}, \dots, EA_{M}\}$. We extend BERT by adding a self-attention mechanism to learn new contextual representations of \emph{Agent A} (denoted as $SA$,) and input text (denoted as $ST$).

\subsection{Final Representation}
We concatenate the lexicon and event-based representation to produce the final representation $CT_{i}$, to be used for argument extraction. 
\begin{equation}
% \small
CT_{i}=LT_{i} \oplus ST_{i} \label{eq:r2}
\end{equation}

==> 5-EventExtraction.tex <==
\section{Ranked Argument Extraction}\label{sec:ArgumentRepresentation}


Given an event type, our argument extraction component aims to generate high-quality dialogue content by ranking the argument extraction order and utilizing the historical dialogue content.
It consists of four main modules: \emph{dialogue generation, argument extraction, incremental event learning, and reinforcement learning based dialogue management}.
The dialogue guided argument extraction model automatically extracts the arguments by inputting the actual event type and text. 
The incremental event learning module then adds the pseudo label as the training data and appends the pseudo-relationship to the lexicon-based graph.
After generating the target sentence's event representation, we follow a dialogue-guided strategy for argument extraction. Specifically, \emph{Agent A} uses the question set from \cite{DBLP:conf/emnlp/DuC20} to generate a query (or question) about an event or a chosen argument (e.g., ``what is the trigger of event \emph{X}?”). Then, \emph{Agent B} answers the query by predicting an argument role or event type. Based on the answer, \emph{Agent A} will then generate a new query in the next turn of argument extraction. This iterative process is driven by an RL-based dialogue management system described in Section \ref{Section 3.3}, aiming to optimize the order of argument extraction. The answer given by \emph{Agent B} will also be fed into an incremental event learning module described later to update the previous answers to be used for the next turn of argument extraction. Later in Table \ref{example}, we give an example dialogue generated by our approach. The automatically generated dialogue produces extra information to be used during the next-turn argument extraction. Our approach is highly flexible, allowing one to tailor the event extraction framework to a specific domain by populating the question set with domain knowledge. 




\subsection{Dialogue Generation}\label{sec:DialogueGeneration}
Our dialogue generation module uses two agents (A and B) to assist event extraction through a sequence of question-answer conversations. Here, \emph{Agent A} generates dialogue content according to the currently processed role.
For each current role, it generates a question set \cite{DBLP:conf/emnlp/DuC20} to create more training data for argument extraction.
\emph{Agent A} produces a hybrid content consisting of both the current argument role and arguments already extracted arguments. 
\emph{Agent B} then generates the content, including the predicted argument given by the argument extraction (described in the next paragraph). 
The predicted argument is then fed into \emph{Agent A} to generate a new dialogue for the next turn of argument extraction. The content of \emph{Agent B} will also be fed into the incremental event learning module described later to add high confidence results for the next turn of argument extraction. 


\subsection{Argument Extraction}
\emph{Agent B} responds to a query by filling the answer slots of a simple answer template designed for each specific question template. It does so by using the learned representation, $CT_{i}$, to locate the start ($i_{s}$) and end ($i_{e}$) position of an argument within the target sentence. Specifically, we obtain the word probability of a chosen argument as:
\begin{equation}
{P}_{start}(r, t, k)=\frac{\exp \left(W^{r s} {CT}_{k}\right)}{\sum_{i=1}^{i=N} \exp \left(W^{r} {CT}_{i}\right)},\label{eq:r10}
\end{equation}
\begin{equation}
{P}_{end}(r, t, k)=\frac{\exp \left(W^{r e} CT_{k}\right)}{\sum_{i=1}^{i=N} \exp \left(W^{r} {CT}_{i}\right)},\label{eq:r11}
\end{equation}
where $W^{r s}$ and $W^{r e}$ are vectors to map ${CT}_{k}$ to a scalar. Each event type $t$ has a type-specific $W^{r s}$ and $W^{r e}$. 
The probability, ${P}_{span}(r, t, a_{i_{s}, i_{e}})$, of an argument being the description (or answer) for argument role $r$ and event type $t$ is given as follows:
\begin{equation}
% \small
{P}_{span}(r, t, a_{i_{s}, i_{e}})={P}_{start}(r, t, i_{s}) \times {P}_{end}(r, t, i_{e}). \label{eq:r12}
\end{equation}


\subsection{Incremental Event Learning}
Our incremental argument learning module tries to incorporate the information obtained at the current argument extraction turn to extract a new argument in the next turn. We do so by adding the extracted argument roles (i.e., pseudo labels) whose reward (evaluated by RL) is greater than a configurable threshold to the input text to provide additional information for extracting new arguments. We also add a new edge (i.e., pseudo relation) to connect the extracted arguments in the lexicon-based graph for an event, so that we can update the lexicon representation to be used for the dialogue in the next turn.  




\subsection{Reinforcement Learning-based Dialogue Management}
\label{Section 3.3}

We use RL to optimize the argument extraction order during our iterative, dialogue-guided argument extraction process. 


\subsubsection{Dialogue Action} 
The dialogue-guided event extraction method defines the action as the set of event schema and argument, which means that the reinforcement learning algorithm needs to decide which argument role to go from the current argument to the following argument.
Different from the previous reinforcement learning-based method, we design two agents with varying spaces of action.
For \emph{Agent A}, action $a_{A}$ is a role from the event schema.
For \emph{Agent B}, action $a_{B}$ is the argument.
Meanwhile, it is necessary to decide whether the current dialogue turn needs to be transferred to the next event type, that is to say, the reinforcement learning algorithm should learn when to switch the event.


\subsubsection{Dialogue State} 
Defined at time step $t$, state $S_{t} \epsilon S$, can be characterized by $S_{t}=(R_{t}, c_{t}^{A}, c_{t}^{B}, Q_{0}, H^{C})$.
Where $R_{t}$ is the argument role selected by the current reinforcement learning algorithm, $c_{t}^{A}, c_{t}^{B}$ are the current embedding of \emph{Agent A} and \emph{B}, $ Q_{0}$ is the initial question of \emph{Agent A} about event type, $H^{C}$ represents the history of the conversation.
Different historical conversation $H^C$ contributes differently to the target argument extraction.
States $s^{A}$ and $s^{B}$ are history-dependent, encoding the historical dialogue and $T$.
$s^{A}$ and $s^{B}$ are the concatenation of the state $s^{A}_{t-1}, s^{B}_{t-1}$ from the last dialogue content and the current content embedding $c^{A}_{t}, c^{B}_{t}$, represented as:
\begin{equation}
\mathrm{s}_{\mathrm{t}}^{A}=\mathrm{s}_{\mathrm{t}-1}^{B} \oplus \mathrm{c}^{A}_{\mathrm{t}},
\end{equation}
\begin{equation}
\mathrm{s}_{\mathrm{t}}^{B}=\mathrm{s}_{\mathrm{t}}^{A} \oplus \mathrm{c}^{B}_{\mathrm{t}}.
\end{equation}



\subsubsection{Dialogue Policy Network} 
The policy is to take correct actions for role selection.
A policy network is a parameterized probability map between action space and degree of belief, which aims to maximize the expected accumulated reward. 

\begin{equation}
% \small
\begin{array}{l}
\pi_{\theta}\left( a^{A}, a^{B} \mid s^{A}, s^{B})\right)= \pi\left(a^{A}, a^{B} \mid (s^{A}, s^{B}); \theta \right)\\
=\mathbb{P}\left(a^{A}_{t}=a^{A}, a^{B}_{t}=a^{B} \mid s^{A}_{t}=s^{A}, s^{B}_{t}=s^{B}, \theta_{t}=\theta\right)
\end{array} \label{eq:r13}
\end{equation}
where $\theta$ is the parameter representing the weight of the policy network. 
The dialogue policy network decides which action should be chosen currently based on the input $T$. It consists of two networks. The first network is the feed-forward network used to encode the conversation history is implemented using a softmax function. The second network is the BiLSTM used to encode the conversation history $H^{C}_{t}=(H^{C}_{t-1},a_{t-1}, s^{A}_{t}, s^{B}_{t})$ as a continuous vector $h^{C}_{t}$, where $H^{C}_{t}$ and $a_{t-1}$ is an observation and action sequence, which is updated by BiLSTM.
\begin{equation}
% \small
e_{T}=\operatorname{softmax}\left(W_{T} F\left(s^{A}, s^{B}\right)+b_{T}\right) \label{eq:r14}
\end{equation}
\begin{equation}
% \small
h^{C}_{t} =BiLSTM\left(h^{C}_{t-1},\left[a_{t-1} ; s^{A}_{t}, s^{B}_{t}\right]\right)  \label{eq:r15}
\end{equation}
where ${W}_{T}$ and ${b}_{T}$ are the parameters, $F\left({s}_{t}\right)$ is the state feature vector, $e_{T}$ is the vector of the input sentence $T$, $a_{t-1}, s^{A}_{t}$ and $s^{B}_{t}$ represent the vector of the action and the current state of \emph{Agent A} and \emph{B} respectively.


\subsubsection{Dialogue Reward} 
The dialogue management module saves the historical dialogues. For the specific event type, the search space is limit. We design a reward function to evaluate all actions. The reward $R(s^{B}, a^{A}, a^{B})$ is defined as the relatedness of the argument extraction part. 
\begin{equation}
% \small
R(s^{B}, a^{A}, a^{B})=\sum_{i}{P}_{span}(r_{i}, t, a_{i_{s}, i_{e}}) \label{eq:r15}
\end{equation}
The policy agent can be effectively optimized using the reward signal. Note that we simultaneously identify all remaining arguments whose reward is less than a threshold in the final turn to avoid error propagation. 







==> 6-EventClassification.tex <==


\section{Event Classification}\label{sec:EventClassification}
  \vspace{-1mm}
Event classification detects whether the input text is an event and classifies the event type to which the text belongs.
In this work, each text is fed into a lexicon-based graph neural network model and an event-based BERT \cite{DBLP:conf/naacl/DevlinCLT19} model to learn the global knowledge and context knowledge of the text, respectively.
The event classification model detects what kinds of events the text contains by adding pseudo argument relation knowledge.
If the text does not contain an event, NULL is output, and the subsequent modules are not executed, enabling it to distinguish the prediction error. 
We use a fully connected layer to compute the context-aware utterance representation $y_{i}$ as follows:
\begin{equation}
% \small
{y}_{i}=ReLU(\boldsymbol{W}({LT}_{i} \oplus {ST}_{i})+b), \label{eq:r3}
\end{equation}
where $\boldsymbol{W}$ and $b$ are trainable parameters, and $\oplus$ denotes vector concatenation operation.
For event classification, a $ReLU$ activation is used to enforce sparsity.
To improve event classification performance,
we design an extra task - predicting the number of event types.
Our multi-task event classification model calculates the combined loss of the two tasks to overcome the event type imbalance results in a low recall.

\subsection{Trigger Classification}


\subsection{Multi-task Joint Loss for Event Classification}
The loss function measures the discrepancy between the predicted value and ground-truth value.
We design two tasks to learn the distinction between prediction error.
For the event classification task, we employ the cross-entropy loss function defined as:
\begin{equation}
% \small
\mathcal{L}_{T} =-\sum_{i} yt_{i} \log \left(\hat{yt}_{i}\right)+(1-yt_{i}) \log \left(1-\hat{yt}_{i}\right), \label{eq:r4}
\end{equation}
where $yt_{i}$ and $\hat{yt}_{i}$ are the $i$-th real label and the predicted label on the event classification task.
For the type number prediction task, we adopt the mean square loss with the $L_{2}$-norm:
\begin{equation}
% \small
\mathcal{L}_{N}=\sum_{i}\left\|\hat{yl}_{i}-yl_{i}\right\|^{2}+\eta\|\Theta\|_{2}, \label{eq:r5}
\end{equation}
where $yl_{i}$ and $\hat{yl}_{i}$ are the $i$-th label and prediction on the second task. $\Theta$ is model parameters, and $\eta$ is a regularization factor.
The overall loss function for optimizing the whole event classification model is:
\begin{equation}
% \small
L=\lambda_{1} L_{T}+\lambda_{2} L_{N}, \label{eq:r6}
\end{equation}
where $\lambda_{1}, \lambda_{2}$ are hyperparameters to balance the two loss.


==> 9-Acknowledgements.tex <==
\section{Acknowledgements}\label{sec:Acknowledgements}
We thank the anonymous reviewers for their insightful comments and suggestions. 
We also would like to thank Yu Hong for providing the ACE2005 corpus.
Work was done when the first author was PhD candidate in Beihang University. 
Jianxin Li is the corresponding author.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

